Fully Dynamic $k$-Clustering in $\tilde O(k)$ Update Time

We present a $O(1)$-approximate fully dynamic algorithm for the $k$-median and $k$-means problems on metric spaces with amortized update time $\tilde O(k)$ and worst-case query time $\tilde O(k^2)$. We complement our theoretical analysis with the first in-depth experimental study for the dynamic $k$-median problem on general metrics, focusing on comparing our dynamic algorithm to the current state-of-the-art by Henzinger and Kale [ESA'20]. Finally, we also provide a lower bound for dynamic $k$-median which shows that any $O(1)$-approximate algorithm with $\tilde O(\text{poly}(k))$ query time must have $\tilde \Omega(k)$ amortized update time, even in the incremental setting.

==> sections/app_algorithm.tex <==
\subsection{Proof of Lemma \ref{lem:bstar}} \label{pf:lm:main:layers}

Consider the ratio $|U_{i+1}|/|U_i|$. Since $U_{i+1} \subseteq U_i$ and $U_{i+1}$ is reconstructed every time $U_i$ is reconstructed, it follows that $|U_{i+1}|/|U_i|$ is at most $(n_{i+1} + \ell) / (n_i + \ell - \ell')$, where $n_j$ is the size of $U_j$ at the time it was last reconstructed and $\ell$ and $\ell'$ are the number of insertions and deletions that have occurred since the last time $U_{i+1}$ was reconstructed respectively. By Lemma \ref{lem:bstar2}, we get that this expression is upper bounded by $(n_{i+1} + \tau n_{i+1})/n_i$. Now we can observe that
\[\frac{|U_{i+1}|}{|U_{i}|} \leq \frac{n_{i+1} + \ell}{n_i + \ell - \ell'} \leq \frac{n_{i+1} + \tau n_{i+1}}{n_i} \leq \frac{n_{i+1}}{n_i} + \tau \leq (1 - \beta) + \epsilon \beta = 1- \beta^*,\]
where we use the facts that $n_{i+1} \leq (1-\beta) n_i$ and $\tau \leq \epsilon \beta$ in the final inequality.

\begin{lemma}\label{lem:bstar2}
Given some integer $i \in [t-1]$, let $\ell$ and $\ell'$ be the number of insertions and deletions that have occurred since the last time $U_{i+1}$ was reconstructed respectively. Then we have that
\[\frac{n_{i+1} + \ell}{n_i + \ell - \ell'} \leq \frac{n_{i+1} + \tau n_{i+1}}{n_i}.\]
\end{lemma}

\begin{proof}
First, note that $(n_{i+1} + \ell)/(n_i + \ell - \ell') \leq (n_{i+1} + \ell)/(n_i - \ell') $. Now, given some reals $A \geq a \geq 0$ and $0 \leq N \leq A -a$, we define a function $f : [0,1] \rightarrow \mathbb R$ by $f(x) = (a + xN)/(A - (1-x)N)$. The derivative of $f$ is $-N(a - A + N)/((x-1)N + A)^2$ and is non-negative for all $x \in [0,1]$. Hence, $f(x) \leq f(1)$ for all $x \in [0,1]$.

By setting $A = n_i$, $a = n_{i+1}$, $N = \ell + \ell'$ and noting that $\ell + \ell' \leq \tau n_{i+1}$ by Invariant \ref{inv:slack} and $n_{i+1} \leq (1- \beta) n_i$, we get that
\[\ell + \ell' \leq \tau n_{i+1} \leq \beta n_{i+1} = (1 + \beta) n_{i+1} - n_{i+1} \leq (1 + \beta)(1 - \beta) n_{i} - n_{i+1} \leq n_{i} - n_{i+1}, \]
and hence it follows that
\[\frac{n_{i+1} + \ell}{n_i - \ell'} = f\left(\frac{\ell}{\ell + \ell'}\right) \leq f(1) = \frac{n_{i+1} + \ell + \ell'}{n_i} \leq \frac{n_{i+1} + \tau n_{i+1}}{n_i}.\]
\end{proof}

\subsection{Proof of Lemma \ref{lem:gamma stability}}\label{pf:lem:gamma stability}

% \begin{lemma}\label{lem:gamma stability app}
% Given a metric subspaces $U_1$ and $U_2$ of $V$ such that $|U_1 \oplus U_2| \leq \frac{\epsilon \gamma}{\gamma(1+\epsilon) + 1} |U_1|$, we have that $\mu_{\gamma}(U_1) \leq 2 \mu_{\gamma(1 + \epsilon)}(U_2)$.
% \end{lemma}

Let $X$ be a subset of $U_2$ of size $k$ such that $\nu_{\gamma(1 + 2\epsilon)}(X, U_2) = \mu_{\gamma(1 + 2\epsilon)}(U_2)$, $\rho = \mu_{\gamma(1 + 2\epsilon)}(U_2)$, and $A = B_{U_1}(X, \rho)$. Now note that
\begin{align*}
    |A| &= |B_{U_1 \cup U_2} (X, \rho) \setminus B_{U_2 \setminus U_1} (X, \rho)|\\
    &\geq |B_{U_2} (X, \rho)| - |B_{U_2 \setminus U_1} (X, \rho)|\\
    &\geq \gamma(1 + 2\epsilon)|U_2| - |U_2 \setminus U_1|\\
    &\geq \gamma(1 + 2\epsilon)|U_2| - \epsilon \gamma |U_1|\\
    &\geq \gamma(1 + 2\epsilon)\left( |U_1| - \epsilon \gamma|U_1| \right) - \epsilon \gamma |U_1|\\
    &= \gamma |U_1| + \epsilon \gamma (1 - \gamma(1 + 2 \epsilon)) |U_1|\\
    &\geq \gamma |U_1|.
\end{align*}
Since there also exists a subset $Y \subseteq A$ of size $k$ such that $A \subseteq B_{U_1}(Y, 2\rho)$, it follows that $\nu_\gamma(Y, U_1) \leq 2\rho$. Hence, $\mu_{\gamma}(U_1) \leq \nu_\gamma(Y, U_1) \leq 2 \mu_{\gamma(1 + 2\epsilon)}(U_2)$.

==> sections/app_time_analysis.tex <==
\begin{lemma}
Each call to \textup{\texttt{Insert}} (Algorithm \ref{alg:insertion}) runs in time $O(\log (|U|/k) \log |U|)$.
\end{lemma}

\begin{proof}
By implementing each of the sets $U_i$ using balanced binary trees, we can insert, delete and check for elements from $U_i$ in worst-case time $O(\log |U_i|)$. Using this implementation, an insertion takes $O(t \log |U|)$ time since we perform $O(t)$ iterations of the loop. Since $t = O(\log (|U|/k))$, our claimed running time follows.
\end{proof}

\begin{lemma}
Each call to \textup{\texttt{Delete}} (Algorithm \ref{alg:deletion}) runs in time $O(\log (|U|/k) \log |U|)$.
\end{lemma}

\begin{proof}
We also implement the $S_i$ and $C_i$ using balanced binary trees to ensure that all operations involving these sets run in time $O(\log |U|)$. Instead of maintaining the assignment $\sigma$ explicitly, we maintain each of the sets in $\Gamma_i = \{ \sigma^{-1}_i(x) \; | \; x \in C_i \}$ for each $i$ such that $0 \leq i \leq t-1$. In other words, we maintain the clustering which partitions $C_i$ at each level. We again implement these as balanced binary trees and also maintain pointers from each $x \in C_i$ to the set (cluster) containing $x$ in $\Gamma_i$. This means that when deleting some $x \in C_i$ we can find the cluster in $\Gamma_i$ containing $x$ in $O(1)$ time and delete $x$ from the cluster. If $x \in S_i$, then we can take any other point in the same cluster as $x$ and place this into $S_i$. If no such other point exists, this cluster is now empty and there is no need to reallocate a center. Note that, since the $C_i$ are disjoint, we only execute lines 5-14 of the algorithm at most once per update. Furthermore, the assignment $\sigma_i$ is maintained implicitly by the collections $\Gamma_i$, so we do not explicitly have to perform the assignment on line 11 of the algorithm.

It follows that each iteration of the loop runs in time $O(\log |U|)$. By the same argument as the preceding lemma, we perform $O(\log(|U|/k))$ many iterations of the loop and our claimed running time follows.
\end{proof}

\begin{lemma}
Each call to \textup{\texttt{ConstructLayer}}$(U')$ (Algorithm \ref{alg:conlayer}) runs in time $O(k' |U'|\log(|U'|))$.
\end{lemma}

\begin{proof}
This follows from the same arguments as in Section 2.1 of \cite{MettuP02} since the construction is the same. It's easy to see that we can also construct the collection of clusters while assigning the points in $U'$ to the sampled centers. However, since $S$, $C$, and the clusters are implemented as balanced binary trees, it takes $O(\log(|U'|))$ to insert the points into the sets, leading to an extra $O(\log(|U'|))$ factor.
\end{proof}

\begin{lemma}
Each call to \textup{\texttt{ReconstructFromLayer}}$(i)$ (Algorithm \ref{alg:reconfromlayer}) runs in time $O(k' |U_i| \log(|U_i|))$.
\end{lemma}

\begin{proof}
This again follows from the same arguments as in Section 2.1 of \cite{MettuP02} since the construction is the same, the only difference being that we again incur an extra $O(\log(|U|))$ factor since we implement the sets a balanced binary trees.
\end{proof}

\begin{lemma}
We can return the weighted instance defined by the assignment $\sigma$ in $\widetilde O(k)$ time.
\end{lemma}

\begin{proof}
First note that $\sigma(U) = (\cup_{i=0}^{t-1} S_i) \cup U_t$, which can easily be computed in $O(|\sigma(U)|)$ time. The weight of each $x \in U_t$ is just $1$. In order to determine the weight of $x \in S_i$ in $O(1)$ time, notice that with the implementation described in the preceding proofs we can use a pointer to find the set $\sigma^{-1}_i(x)$ in $O(1)$ time, which is implemented as a balanced binary tree. By implementing a counter for the number of elements contained within the tree, we can find $|\sigma^{-1}_i(x)|$ in $O(1)$ time. Since $|\sigma(U)| = O(k't)$ and $t = \widetilde O(1)$, this can be done in $\widetilde O(k)$ time.
\end{proof}

==> sections/approx_analysis.tex <==
In this section we fix a value $\gamma$ such that $\beta < \gamma < 1$ and reconstruction factor $\epsilon$ such that $0 < \epsilon < \min \{\frac{1}{\gamma} - 1, 1 \}$. We also define $k'$ to be the maximum of $k$ and $\log (|U|)$ and $\tau$ to be  $\frac{\epsilon\beta}{\beta(1 + \epsilon) + 1}$. Note that the value of $k'$ can change as points are inserted and deleted.

Consider the state of our dynamic algorithm after being initialized and handling some arbitrary sequence of updates. We now show that, with high probability, $\cost(\sigma) = O(\textsc{opt}_k)$, where $\sigma$ is the assignment currently maintained by our dynamic algorithm and $\textsc{opt}_k$ denotes the value of an optimal solution to the $k$-medians problem on the current input $U$.

Let $U = U_0 \supseteq ... \supseteq U_t$ denote the layers currently maintained by our algorithm and let $U^{\textsc{old}}_i$ denote the state of the $i$th layer the last time it was reconstructed for $0 \leq i \leq t-1$. 

\subsection{Bounding the Radii $\nu_i$}\label{sec:bound nu}

In this subsection we use the following crucial lemma which is analogous to Lemma 4.3.3 in \cite{Mettu02}. The changes required to turn the proof of Lemma 4.3.3 in \cite{Mettu02} into a proof for Lemma \ref{lem:MP nu bound} are trivial.

\begin{lemma}\label{lem:MP nu bound}
Given any positive $\xi$, there exists a sufficiently large choice of $\alpha$ such that $\nu_i \leq 2 \mu_\gamma(U^{\textsc{old}}_i)$ for each $0 \leq i \leq t-1$ with probability at least $1 - e^{-\xi k'}$.
\end{lemma}

% \begin{lemma}
% Given any positive $\xi$, there exists a sufficiently large choice of $\alpha$ such that the value $\nu$ computed by calling \textup{\texttt{ConstructLayer}} (Algorithm \ref{alg:conlayer}) on input $U$ satisfies $\nu \leq 2 \mu_\gamma(U)$ with probability at least $1 - e^{-\xi k'}$.
% \end{lemma}

\noindent
From now on we fix some positive $\xi$ and sufficiently large $\alpha$ such that the statement of Lemma \ref{lem:MP nu bound} holds. Let $\gamma^*$ and $\beta^*$ denote $\gamma(1 + \epsilon)$ and $\beta(1-\epsilon)$ respectively.

\begin{lemma}\label{lem:our nu bound}
$\nu_i \leq 4 \mu_{\gamma^*}(U_i)$ for each $0 \leq i \leq t-1$ with probability at least $1 - e^{-\xi k'}$.
\end{lemma}

\begin{proof}
For each $0 \leq i \leq t-1$, $|U_i \oplus U^{\textsc{old}}_i| \leq \tau |U^{\textsc{old}}_i|$ since at most $\tau |U^{\textsc{old}}_i|$ points have been inserted or deleted from $U_i$ since it was last reconstructed. Noticing that $\beta < \gamma$ and $\tau$ is increasing as a function of $\beta$ we can see that
\[|U_i \oplus U^{\textsc{old}}_i| \leq \frac{\epsilon \gamma}{\gamma(1+\epsilon) + 1} |U^{\textsc{old}}_i|.\]
Applying Lemma \ref{lem:gamma stability} it follows that $\mu_\gamma(U^{\textsc{old}}_i) \leq 2 \mu_{\gamma^*}(U_i)$. The lemma follows by combining this result with Lemma \ref{lem:MP nu bound}.
\end{proof}

\subsection{Upper Bounding the Cost}\label{sec:upper bound cost}

\begin{lemma}\label{upperbndcost1}
For all $i$ such that $0 \leq i \leq t-1$, $\cost(\sigma, C_i) \leq 2 \nu_i |C_i|$.
\end{lemma}

\begin{proof}
Each point $x$ in $C_i$ is assigned to some point $y \in C_i$ such that $d(x, y) \leq 2 \nu_i$.
\end{proof}

\begin{lemma}\label{upperbndcost2}
\[\cost(\sigma) \leq \sum_{i=0}^{t-1} 2\nu_i |C_i|.\]
\end{lemma}

\begin{proof}
Follows directly from the fact that the $C_i$ partition $U$, Lemma \ref{upperbndcost1}, and the fact that $\cost(\sigma, C_t) = 0$.
\end{proof}

\subsection{Lower Bounding the Cost}

Let $r$ denote $\lceil \log_{1-\beta^*} \frac{1-\gamma^*}{3} \rceil$ and for each $0 \leq i \leq t-1$ let $\mu_i$ denote $\mu_{\gamma^*}(U_i)$. We now prove the following lemma which immediately gives a lower bound on $\textsc{opt}_k$.

\begin{lemma}
Given any $S \subseteq U$ of size $k$, we have that
\[\cost(S) \geq \frac{1-\gamma^*}{2r} \sum_{i=1}^{t-1} \mu_i |C_i|.\]
\end{lemma}

\noindent
For the rest of this subsection we fix an arbitrary $S \subseteq U$ of size $k$. For each $0 \leq i \leq t-1$, let $F_i$ denote the set $\{x \in U_i \; | \; d(x,S) \geq \mu_i\}$, and for any integer $m > 0$, let $F_i^m$ denote $F_i \setminus (\cup_{j > 0} F_{i + jm})$ and $G_{i,m}$ denote the set of all integers $j$ such that $0 \leq j \leq t-1$ and $j \equiv i \pmod{m}$.

The following lemma is proven in \cite{Mettu02}.

\begin{lemma}[\cite{Mettu02}, Lemma 4.3.6]\label{lowerbound1}
Given integers $\ell$ and $m > 0$ such that $0 \leq \ell \leq t-1$, and $i, j \in G_{l,m}$ such that $i \neq j$, we have that $F^m_i \cap F^m_j = \varnothing$.
\end{lemma}

\begin{lemma}\label{lowerbound2}
Given some integer $i$ such that $0 \leq i \leq t-1$ and a subset $X \subseteq F_i$, we have that $|F_i| \geq (1-\gamma^*) |U_i|$ and $\cost(S,X) \geq \mu_i |X|$.
\end{lemma}

\begin{proof}
It follows directly from the definition of $\mu_i$ that we have that $|F_i| \geq (1 - \gamma^*)|U_i|$. By the definition of $F_i$, we have that $\cost(S,X) = \sum_{x \in X} d(x,S) \geq \mu_i |X|$.
\end{proof}

The following lemma is proven in \cite{Mettu02}.

\begin{lemma}[\cite{Mettu02}, Lemma 4.3.8]\label{lowerbound3}
Given integers $\ell$ and $m > 0$ such that $0 \leq \ell \leq t-1$, we have that
\[\cost(S, \cup_{i \in G_{\ell, m}} F^m_i) \geq \sum_{i \in G_{\ell, m}} \mu_i |F^m_i|.\]
\end{lemma}

The proof of the following lemma is given in Appendix \ref{app:approx_analysis}.

\begin{lemma}\label{lem:bstar}
For all $i$ such that $0 \leq i \leq t-2$, we have that $|U_{i+1}| \leq (1 - \beta^*) |U_i|$.
\end{lemma}

\begin{lemma}\label{lowerbound4}
For all $i$ such that $0 \leq i \leq t-1$, we have that $|F_{i+r}| \leq \frac{1}{3}|F_i|$.
\end{lemma}

\begin{proof}
This follows from the fact that
\begin{multline*}
|F_{i+r}| \leq |U_{i+r}| \leq (1-\beta^*)^r|U_i| \\ \leq \frac{(1-\beta^*)^r}{1-\gamma^*}|F_i| \leq \frac{1}{3}|F_i|.
\end{multline*}
The first inequality follows from the fact that $F_{i+r} \subseteq U_{i+r}$, the second inequality follows from Lemma \ref{lem:bstar}, the third inequality follows from Lemma \ref{lowerbound2}, and the fourth inequality follows from the definition of $r$.
\end{proof}

\begin{lemma}\label{lowerbound5}
For all $i$ such that $0 \leq i \leq t-1$, we have that $|F^r_i| \geq \frac{1}{2}|F_i|$.
\end{lemma}

\begin{proof} This follows from the fact that
\begin{multline*}
|F^r_i| = |F_i \setminus \cup_{j > 0}F_{i + jr} | \geq |F_i| - \sum_{j > 0} \frac{1}{3^j}|F_i| \geq \frac{1}{2}|F_i|.
\end{multline*}
\end{proof}

\begin{lemma}\label{lowerbound6}
\[\cost(S) \geq \frac{1-\gamma^*}{2r} \sum_{i=1}^{t-1} \mu_i|C_i|. \]
\end{lemma}

\begin{proof}
Let $\ell = \arg \max_{0 \leq \ell < r} \{\sum_{i \in G_{\ell, r}} \mu_i |F^r_i|\}$. Then we have that
\begin{align*}
    \cost(S) &\geq \cost(S, \cup_{i \in G_{\ell, r}} F^r_i)\\
    		&\geq \sum_{i \in G_{\ell, r}} \mu_i |F^r_i|\\
		&\geq \frac{1}{r} \sum_{i =0}^{t-1} \mu_i |F^r_i|\\
		&\geq \frac{1}{2r} \sum_{i =0}^{t-1} \mu_i |F_i|\\
		&\geq \frac{1 - \gamma^*}{2r} \sum_{i =0}^{t-1} \mu_i |U_i|\\
		&\geq \frac{1 - \gamma^*}{2r} \sum_{i =0}^{t-1} \mu_i |C_i|.
\end{align*}
The second inequality follows from Lemma \ref{lowerbound3}, the third inequality from averaging and the choice of $\ell$, the fourth inequality from Lemma \ref{lowerbound5}, and the fifth inequality from Lemma \ref{lowerbound2}.
\end{proof}

\subsection{Approximation Ratio}

It follows that with probability at least $1 - e^{-\xi k'}$ we have that
\[\cost(\sigma) \leq \sum_{i=1}^{t-1} 2\nu_i |C_i| \leq \sum_{i=1}^{t-1} 8\mu_i |C_i| \leq \frac{16r}{1-\gamma^*} \cost(S)\]
for any set $S \subseteq U$ of size $k$. Hence, we have that
\[\cost(\sigma) \leq \frac{16r}{1-\gamma^*} \textsc{opt}_k.\]
In particular, the assignment $\sigma$ is a $O(1)$-approximation to the optimal solution.

==> sections/lower_bounds.tex <==


The following lower bound is proven by Mettu in \yrcite{Mettu02}. Informally, the proof of this lower bound is obtained by constructing, for each $\delta > 0$, an input distribution of metric spaces (with polynomially bounded aspect ratio) on which no deterministic algorithm for the $k$-median problem succeeds with probability more than $\delta$. Theorem~\ref{thm:mettu:lb} then follows by an application of Yao's minmax principle.

\begin{theorem}\label{thm:mettu:lb}
Any $O(1)$-approximate randomized (static) algorithm for the $k$-median problem, which succeeds with even negligible probability, runs in time $\Omega(nk)$.
\end{theorem}

Note that any incremental algorithm for $k$-median with amortized update time $u(n,k)$ and query time $q(n,k)$ can be used to construct a static algorithm for the $k$-median problem with running time $n \cdot u(n,k) + q(n,k)$ by inserting each point in the input metric space $U$ followed by a solution query. Hence, by Theorem~\ref{thm:mettu:lb}, we must have that $n \cdot u(n,k) + q(n,k) = \Omega(nk)$. Now assume that some incremental algorithm for $k$-median has query time $\tilde O(\poly(k))$. If this algorithm also has an amortized update time of $\tilde o(k)$, then for the range of values of $k$ where $q(n,k) = \tilde o(n)$, it follows that $\tilde o(nk) + \tilde o(n)$ is $\Omega(nk)$, giving a contradiction. Hence, the amortized update time must be $\tilde \Omega(nk)$ and \ref{thm:OurLBapp} follows.

\begin{theorem}\label{thm:OurLBapp}
Any $O(1)$-approximate randomized incremental algorithm for the $k$-median problem with $O(\poly(k))$ query time must have $\tilde \Omega(nk)$ amortized update time.
\end{theorem}

==> sections/time_analysis.tex <==
We now proceed to bound the amortized update time of our algorithm. If we ignore the time taken while handling a call to the function \texttt{Reconstruct}, an update can easily be implemented to run in time $\widetilde O(1)$. We formalize this with Lemma \ref{lem:insertion} and Lemma \ref{lem:deletion}. The proofs of these lemmas follow from standard implementations. By then showing that the total running time of calls to the function \texttt{Reconstruct} during an update stream of length $m$ is $\widetilde O(mk)$, it follows that the amortized update time of our algorithm is $\widetilde O(k)$.

This follows from a charging scheme. We prove this by first showing that each call to \texttt{ReconstructFromLayer}$(i)$ can be implemented to run in time $O(|U_i|k')$, and then \textit{charging} the cost of this computation to the $\Omega (|U_i|)$ many updates that have occurred since the last time this layer was reconstructed, with each update being charged a cost of $O(k' \log(|U|))$. By then showing that each update is charged at most $\widetilde O(1)$ times, the amortized guarantee follows.

In order to prove the following lemmas, we crucially use the fact that the number of layers in our data structure, $t$, is $O(\log (|U|/k))$. We later show in Lemma \ref{lem:bstar} that the sizes of these layers do indeed decrease exponentially. combining this with the fact that $|U_{t-1}| = \Omega(k)$, the bound on $t$ follows. The proofs of the following lemmas have all been deferred to Appendix \ref{app:time_analysis}.

\begin{lemma}\label{lem:insertion}
Each call to \textup{\texttt{Insert}} (Algorithm \ref{alg:insertion}) runs in time $O(\log (|U|/k) \log |U|)$.
\end{lemma}

\begin{lemma}\label{lem:deletion}
Each call to \textup{\texttt{Delete}} (Algorithm \ref{alg:deletion}) runs in time $O(\log (|U|/k) \log |U|)$.
\end{lemma}

% \begin{lemma}\label{lem:conlayer}
% Each call to \textup{\texttt{ConstructLayer}}$(U')$ (Algorithm \ref{alg:conlayer}) runs in time $O(k |U'|)$.
% \end{lemma}

\begin{lemma}\label{lem:reconlayer}
Each call to \textup{\texttt{ReconstructFromLayer}}$(i)$ (Algorithm \ref{alg:reconfromlayer}) runs in time $O(k' |U_i| \log(|U_i|))$.
\end{lemma}

Now note that each update can only be charged for at most $t = O(\log(|U|/k))$ different calls to the function \textup{\texttt{ReconstructFromLayer}}. This is because the reconstructions at layer $i$ can only charge each update at most once. Since the cost incurred by an update each time it gets charged is $O(k'\log(|U|))$, it follows that each update gets charged a cost of at most $O(k' \log(|U|) \log(|U|/k))$. Note that $|U|$, and hence $t$, will only change by a small constant multiplicative factor between full reconstructions of the entire data structure. Hence, the amortized update time of our algorithm is $O((k + \log(|U|))\log(|U|)\log(|U|/k))$.

\begin{theorem}
Our dynamic algorithm has an amortized update time of $\widetilde O(k)$.
\end{theorem}
